A Tightly Coupled LiDAR-IMU Odometry through Iterated Point-Level Undistortion

Scan undistortion is a key module for LiDAR odometry in high dynamic environment with high rotation and translation speed. The existing line of studies mostly focuses on one pass undistortion, which means undistortion for each point is conducted only once in the whole LiDAR-IMU odometry pipeline. In this paper, we propose an optimization based tightly coupled LiDAR-IMU odometry addressing iterated point-level undistortion. By jointly minimizing the cost derived from LiDAR and IMU measurements, our LiDAR-IMU odometry method performs more accurate and robust in high dynamic environment. Besides, the method characters good computation efficiency by limiting the quantity of parameters.

==> src/02-rw.tex <==
\newcommand{\DALLE}{{DALL$\cdotBB$E}}

\section{Related Work}\label{sec:rw}
